The Impact of Surface Passivation on Kapitza Resistance at the Interface between a Semiconductor and Liquid Nitrogen

Cooling electronic devices to cryogenic temperatures (< 77 K) is crucial in various scientific and engineering domains. Efficient cooling involves the removal of heat generated from these devices through thermal contact with either a liquid cryogen or a dry cryostat cold stage. However, as these devices cool, thermal boundary resistance, also known as Kapitza resistance, hinders the heat flow across thermal interfaces, resulting in elevated device temperatures. In transistors, the presence of passivation layers like Silicon Nitride (SiN) introduces additional interfaces that further impede heat dissipation. This paper investigates the impact of passivation layer thickness on Kapitza resistance at the interface between a solid device and liquid nitrogen. The Kapitza resistance is measured using a capacitance thermometer that has been passivated with SiN layers ranging from 0 to 240 nm. We observe that Kapitza resistance increases with increasing passivation thickness.

==> note.tex <==
|%Another important consideration in understanding heat transfer at the interface is the diffuse mismatch theory \cite{b211} which is related to  phonon scattering at the interface due to their wavelength. %The effect of phonon wavelength on Kapitza resistance is such that larger wavelengths promote more efficient heat transfer.\\
%When the phonon wavelength is much larger than the characteristic dimensions of the interface, such as the inter-atomic spacing or the thickness of the interface region, the phonons tend to propagate relatively freely across the interface. This results in a lower Kapitza resistance as the phonons can efficiently transfer heat. However, smaller wavelengths introduce greater resistance. When the phonon wavelength becomes comparable to or smaller than the characteristic dimensions of the interface, phonon scattering and reflection at the interface become more significant. This leads to increased resistance to phonon transport and, consequently, a higher Kapitza resistance \cite{b20},\cite{b22,b233,b234}. \\ %We estimate that this passivation layer acts as a reflective coating layer for phonons, and characterizing the passivation layer thickness to achieve minimum Kapitza resistance leads to better heat dispersion. The results can then be applied to low-noise electronics such as  HEMT-based amplifiers to study noise behavior.\\ 
%Further, Considering  \cite{b23} and \cite{b24},   
%table \ref{tab:PhononWavelength} provides the range of dominant phonon wavelength at different temperatures for the applied materials in this experiment.
%\begin{table}[h!]
%\caption{Dominant phonon wavelength}
%\label{tab:PhononWavelength}
%\centering
%\renewcommand{\arraystretch}{1.5}
%\begin{tabular}{lcc}
%\hline
%Material & \multicolumn{2}{c}{Wavelength (nm)} \\

 %& 300K&77K \\
%\hline
%\hline
%Au &0.152-0.226&0.89-72.6 \\
%SiN &0.314-66.78 &0.1430- \\
%\hline
%\end{tabular}
%\end{table}%


%It can be anticipated that the passivation layer thickness should be in the range or lower than that of the phonon wavelength provided in table \ref{tab:PhononWavelength} to improve the thermal dissipation.\\

